MOODv2: Masked Image Modeling for Out-of-Distribution Detection

The crux of effective out-of-distribution (OOD) detection lies in acquiring a robust in-distribution (ID) representation, distinct from OOD samples. While previous methods predominantly leaned on recognition-based techniques for this purpose, they often resulted in shortcut learning, lacking comprehensive representations. In our study, we conducted a comprehensive analysis, exploring distinct pretraining tasks and employing various OOD score functions. The results highlight that the feature representations pre-trained through reconstruction yield a notable enhancement and narrow the performance gap among various score functions. This suggests that even simple score functions can rival complex ones when leveraging reconstruction-based pretext tasks. Reconstruction-based pretext tasks adapt well to various score functions. As such, it holds promising potential for further expansion. Our OOD detection framework, MOODv2, employs the masked image modeling pretext task. Without bells and whistles, MOODv2 impressively enhances 14.30% AUROC to 95.68% on ImageNet and achieves 99.98% on CIFAR-10.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> algorithms/moodv1.tex <==
%--------------------------------------algorithm-----------------------------------
\begin{algorithm*}[t!]
\caption{Masked Image Modeling Out-of-distribution Detection Algorithm}
\label{alg1}
\small
\begin{algorithmic}[1]

\Require Pre-train set $X_P$, in-distribution set $X_{\rm ID}$, test set $X_{\rm test}$, required True Positive Rate $\eta$\%.
\Ensure Is $x_{\rm test}$ outlier or not? $\forall x_{\rm test} \in X_{\rm test}$.

% \State\textbf{Function} $d(z, \mu, \sum)$: 
% $$ d(z, \mu, \sum)=\left [(z-\mu)^T{\textstyle \sum^{-1}}(z-\mu) \right ] $$

\State Partition $X_{\rm ID}$ into the training set $X_{\rm train}$ and calibration set $X_{\rm cal}$. 
\State Pre-train $f_{\rm ViT}$ on $X_P$ by maximizing
$$\sum_{x\in X_P}\mathbb{E}_M\left [\sum_{i\in M}\log p_{\rm MIM}(z|x^M)\right ]$$.
\State Intermediately Fine-tune $f_{\rm ViT}$ on $X_P$ by minimizing {\color{gray}\Comment{Not for one-class OOD detection except on ImageNet-30.}}
$$L_{\rm interft}=\sum_{x_p\in X_P}{\rm CrossEntropy}(f_{\rm ViT}(x_p), y_P(x_p))$$ 
\State Fine-tune $f_{\rm ViT}$ on $X_{\rm train}$ by minimizing  {\color{gray}\Comment{Not for one-class OOD detection on ImageNet-30.}} 
$$L_{\rm train}=\sum_{x\in X_{\rm train}}{\rm CrossEntropy}(f_{\rm ViT}(x), y^{LS}(x))$$ 
where $y^{LS}$ is defined by $$y_c^{LS} = y_c(1-\alpha)+\alpha/N_c, \quad\quad c=1, 2, \dots, N_c$$
where $c$ is the index of category; $N_c$ is the number of classes; and $\alpha$ is the hyperparameter that determines smoothing level.
\State $h(x)=f_{\rm ViT}(x)$ for $x \in X_{\rm train} \cup X_{\rm test} \cup X_{\rm cal}$. 
% \State $h(X_{\rm train})=f_{\rm ViT}(X_{\rm train})$.
%\State $\mu=\sum_{x\in X_{\rm train}}(h(x))$
%\State $\sum=\sqrt{\frac{1}{N}(h(x)-\mu)}$ 
%\State $h(X_{\rm test})=f_{\rm ViT}(X_{\rm test})$.
%\State $h(X_{\rm cal})=f_{\rm ViT}(X_{\rm cal})$.
\State Use $h(x)$ to calculate $d(x_{\rm test})$ for $x_{\rm test} \in X_{\rm test}$ and $d(x_{\rm cal})$ for $x_{\rm cal}\in X_{\rm cal}$, where $d(\cdot)$ is defined by $$d_2(x)=\left [(h(x)-\mu)^T{\textstyle \sum^{-1}}(h(x)-\mu) \right ]$$
where $\mu$ and $\sum$ are the mean and covariance of the encoding vectors $h(x)$ of the ID training set $X_{\rm train}$.
%\State Compute $d(x_{\rm test}\in X_{\rm test})$ and $d(x_{\rm cal}\in X_{\rm cal})$, where $d(\cdot)$ is defined by \cref{equ:distance}.
%\State Compute $d(x)$ for $x \in X_{\rm cal}, \cupX_{\rm test}$, where $d(x)$ is defined by \cref{equ:distance}.
\State Compute threshold $T$ as the $\eta$ percentile of $d(x_{\rm cal})$.
% \If {$d(x_{\rm test})>(d(x_{\rm cal})$ at threshold at TPR)}
\If {$d(x_{\rm test})>T$}
\State $x_{\rm test}$ is an outlier.
\EndIf
\end{algorithmic}
\end{algorithm*}

==> tables/difference.tex <==
\iffalse
\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{0.5mm}
\begin{tabular}{c|cccccccccc|c}
\toprule
Datasets & ImageNet & Texture & iNaturalist & ImageNet-O & OpenImage-O \\
\midrule
Distance & 18.09 & 32.89 & 38.96 & 30.76 & 45.56 \\
\bottomrule
\end{tabular}
\caption{\textbf{Difference.} .}
\label{tab:difference}
\end{table}
\fi 

\begin{table}[t]
\small
\centering
\setlength{\tabcolsep}{3mm}
\begin{tabular}{c|cc}
\toprule
ID/OOD & Datasets & Recovery Distance \\
\midrule
ID & ImageNet (ID) \cite{imagenet} & \revise{18.09} \\
\midrule
\multirow{4}{*}{OOD} & Texture \cite{dtd} & \revise{32.89} \\
& INaturalist \cite{inaturalist}& \revise{38.96} \\
& ImageNet-O \cite{imagenet_o} & \revise{30.76} \\
& OpenImage-O \cite{openimages_o} & \revise{45.56} \\
\bottomrule
\end{tabular}
\caption{\revise{The average recovery distance (L2 norm between the original images and their corresponding reconstructions) for ID and OOD datasets. For each dataset, the number of sampled images is the minimum of 5000 and the dataset size.}}
\label{tab:difference}
\end{table}

==> tables/mim-imagenet-avgood.tex <==
%%%%%%%%%%%%%%% one tables %%%%%%%%%%%%%%%
\begin{table*}[t]
\small
\centering
\subfloat[AUROC]{
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{c|cccccccccccc}
\toprule
% Models & MSP\cite{baseline_ood} & Energy\cite{energy} & MaxLogit\cite{maxlogit} & KL-Matching\cite{maxlogit} & Residual & React\cite{react} & Mahalanobis\cite{mahalanobis} & ViM\cite{vim} & Best \\
Models & MSP & Energy & MaxLogit & KL-Matching & Residual & Energy+React & Mahalanobis & ViM & Average & Best \\
\midrule
ViT\cite{vit} & 76.77 & 65.85 & 75.37 & 80.28 & 74.86 & 74.34 & 81.38 & 77.65 & 75.81 & 81.38 \\
MoCov3\cite{mocov3} & 76.94 & 65.57 & 75.64 & 79.78 & 68.64 & 67.61 & 81.28 & 72.07 & 73.44 & 81.28 \\
DINOv2\cite{dinov2} & 51.83 & 65.21 & 56.20 & 67.46 & 61.04 & 67.60 & 62.04 & 61.32 & 61.59 & 67.60 \\
\rowcolor{gray!20}BEiTv2\cite{beitv2} & 88.83 & \textbf{90.42} & \textbf{90.16} & 89.31 & 94.17 & \textbf{91.21} & 93.51 & 95.42 & 91.63 & 95.42 \\
\rowcolor{gray!20}BEiT\cite{beit} & \textbf{89.00} & 89.85 & 89.83 & \textbf{89.93} & \textbf{94.88} & 90.64 & \textbf{94.39} & \textbf{95.68} & \textbf{91.77} & \textbf{95.68} \\
MaskFeat\cite{maskfeat} & 33.86 & 59.86 & 34.26 & 55.00 & 74.04 & 55.10 & 85.46 & 74.12 & 58.96 & 85.46 \\
EVA\cite{eva} & 48.99 & 63.10 & 49.67 & 67.49 & 72.43 & 51.72 & 83.83 & 72.52 & 63.72 & 83.83 \\
MFF\cite{mff} & 50.36 & 57.19 & 50.64 & 44.90 & 64.49 & 50.28 & 50.70 & 64.56 & 54.14 & 64.56 \\
MILAN\cite{milan} & 43.81 & 39.16 & 41.84 & 67.68 & 70.94 & 39.74 & 71.65 & 70.25 & 55.63 & 71.65 \\
CAE\cite{cae} & 62.32 & 52.12 & 62.23 & 46.81 & 50.95 & 51.44 & 50.94 & 51.02 & 53.48 & 62.32 \\
\bottomrule
\end{tabular}
\label{tab:multi-imagenet-avgood-auroc}
}

\subfloat[FPR95]{
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{c|cccccccccccc}
\toprule
% Models & MSP\cite{baseline_ood} & Energy\cite{energy} & MaxLogit\cite{maxlogit} & KL-Matching\cite{maxlogit} & Residual & React\cite{react} & Mahalanobis\cite{mahalanobis} & ViM\cite{vim} & Best \\
Models & MSP & Energy & MaxLogit & KL-Matching & Residual & Energy+React & Mahalanobis & ViM & Average & Best \\
\midrule
ViT\cite{vit} & 68.30 & 78.49 & 68.67 & 74.84 & 79.01 & 65.15 & 77.80 & 76.40 & 73.58 & 65.15 \\
MoCov3\cite{mocov3} & 64.45 & 76.75 & 63.93 & 78.89 & 84.61 & 75.16 & 78.81 & 82.54 & 75.64 & 63.93 \\
DINOv2\cite{dinov2} & 93.44 & 77.13 & 90.26 & 82.59 & 87.24 & 81.17 & 86.93 & 87.04 & 85.72 & 77.13 \\
\rowcolor{gray!20}BEiTv2\cite{beitv2} & 39.25 & \textbf{28.85} & 32.37 & 43.47 & 27.52 & \textbf{27.52} & 31.60 & 22.95 & 31.69 & 22.95 \\
\rowcolor{gray!20}BEiT\cite{beit} & \textbf{38.60} & 29.01 & \textbf{31.47} & \textbf{42.54} & \textbf{24.49} & 28.17 & \textbf{26.92} & \textbf{20.22} & \textbf{30.18} & \textbf{20.22} \\
MaskFeat\cite{maskfeat} & 98.80 & 92.26 & 98.71 & 89.33 & 81.84 & 94.52 & 71.07 & 81.76 & 88.54 & 71.07 \\
EVA\cite{eva} & 95.87 & 89.18 & 95.71 & 76.51 & 71.76 & 94.20 & 62.47 & 71.71 & 82.18 & 62.47 \\
MFF\cite{mff} & 94.80 & 95.76 & 94.67 & 92.63 & 79.89 & 97.64 & 94.54 & 79.87 & 91.22 & 79.87 \\
MILAN\cite{milan} & 95.17 & 94.45 & 95.30 & 82.05 & 77.95 & 94.31 & 77.77 & 79.06 & 87.01 & 77.77 \\
CAE\cite{cae} & 86.06 & 94.45 & 86.19 & 95.58 & 95.24 & 93.88 & 95.04 & 95.24 & 92.71 & 86.06 \\
\bottomrule
\end{tabular}
\label{tab:multi-imagenet-avgood-fpr50}
}
\caption{\textbf{Multi-Class OOD Detection on ImageNet.} Performance of multi-class OOD Detection on ImageNet.}
\label{tab:multi-cifar10-avgood}
\end{table*}

==> tables/mim-imagenet-detailed.tex <==
%--------------------------------------multi-class-----------------------------------
\begin{table*}[tp]
\small
\centering
\setlength{\tabcolsep}{0.5mm}
\begin{tabular}{c|c|cccccccccc}
\toprule
\multirow{2}{*}{Methods} & \multirow{2}{*}{Models} & \multicolumn{2}{c}{Texture} & \multicolumn{2}{c}{iNaturalist} & \multicolumn{2}{c}{ImageNet-O} & \multicolumn{2}{c}{OpenImage-O} & \multicolumn{2}{c}{Average} \\
& & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ \\
\midrule
\multirow{10}{*}{MSP\cite{baseline_ood}}
& ViT\cite{vit} & 71.31 & 77.07 & 90.70 & 43.72 & 60.77 & 90.60 & 84.29 & 61.79 & 76.77 & 68.30 \\
& MoCov3\cite{mocov3} & 66.85 & 76.24 & 90.68 & 42.03 & 64.80 & 84.60 & 85.42 & 54.94 & 76.94 & 64.45 \\
& DINOv2\cite{dinov2} & 47.49 & 91.74 & 62.13 & 92.36 & 44.87 & 95.60 & 52.83 & 94.04 & 51.83 & 93.44 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{\textbf{85.61}} & \cellcolor{gray!20}{51.45} & \cellcolor{gray!20}{\textbf{96.05}} & \cellcolor{gray!20}{\textbf{16.89}} & \cellcolor{gray!20}{81.15} & \cellcolor{gray!20}{58.30} & \cellcolor{gray!20}{\textbf{92.52}} & \cellcolor{gray!20}{\textbf{30.34}} & \cellcolor{gray!20}{88.83} & \cellcolor{gray!20}{39.25} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{85.05} & \cellcolor{gray!20}{\textbf{48.80}} & \cellcolor{gray!20}{95.50} & \cellcolor{gray!20}{19.56} & \cellcolor{gray!20}{\textbf{83.17}} & \cellcolor{gray!20}{\textbf{54.95}} & \cellcolor{gray!20}{92.28} & \cellcolor{gray!20}{31.10} & \cellcolor{gray!20}{\textbf{89.00}} & \cellcolor{gray!20}{\textbf{38.60}} \\
& MaskFeat\cite{maskfeat} & 29.63 & 98.88 & 31.02 & 99.61 & 37.87 & 98.05 & 36.91 & 98.67 & 33.86 & 98.80 \\
& EVA\cite{eva} & 38.58 & 97.15 & 59.85 & 93.50 & 47.59 & 96.65 & 49.94 & 96.16 & 48.99 & 95.87 \\
& MFF\cite{mff} & 42.84 & 96.18 & 49.63 & 95.76 & 51.81 & 94.40 & 57.17 & 92.84 & 50.36 & 94.80 \\
& MILAN\cite{milan} & 42.28 & 93.95 & 32.03 & 99.70 & 56.72 & 92.10 & 44.21 & 94.93 & 43.81 & 95.17 \\
& CAE\cite{cae} & 59.23 & 88.00 & 70.37 & 79.43 & 57.94 & 90.10 & 61.74 & 86.72 & 62.32 & 86.06 \\
\midrule
\multirow{10}{*}{Energy\cite{energy}}
& ViT\cite{vit} & 54.11 & 86.28 & 76.61 & 72.70 & 61.63 & 81.00 & 71.06 & 73.99 & 65.85 & 78.49 \\
& MoCov3\cite{mocov3} & 48.79 & 88.33 & 76.80 & 73.09 & 64.56 & 75.60 & 72.13 & 69.99 & 65.57 & 76.75 \\
& DINOv2\cite{dinov2} & 73.89 & 68.16 & 80.34 & 59.18 & 49.98 & 94.15 & 56.64 & 87.03 & 65.21 & 77.13 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{\textbf{85.32}} & \cellcolor{gray!20}{\textbf{44.15}} & \cellcolor{gray!20}{\textbf{96.95}} & \cellcolor{gray!20}{\textbf{10.67}} & \cellcolor{gray!20}{85.27} & \cellcolor{gray!20}{40.95} & \cellcolor{gray!20}{\textbf{94.14}} & \cellcolor{gray!20}{\textbf{19.62}} & \cellcolor{gray!20}{\textbf{90.42}} & \cellcolor{gray!20}{\textbf{28.85}} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{83.04} & \cellcolor{gray!20}{44.59} & \cellcolor{gray!20}{96.48} & \cellcolor{gray!20}{12.42} & \cellcolor{gray!20}{\textbf{86.36}} & \cellcolor{gray!20}{\textbf{37.85}} & \cellcolor{gray!20}{93.50} & \cellcolor{gray!20}{21.18} & \cellcolor{gray!20}{89.85} & \cellcolor{gray!20}{29.01} \\
& MaskFeat\cite{maskfeat} & 61.42 & 91.53 & 54.38 & 96.50 & 62.56 & 89.70 & 61.10 & 91.32 & 59.86 & 92.26 \\
& EVA\cite{eva} & 59.29 & 82.79 & 64.58 & 94.94 & 63.79 & 89.15 & 64.74 & 89.85 & 63.10 & 89.18 \\
& MFF\cite{mff} & 48.25 & 96.41 & 71.22 & 94.05 & 48.84 & 97.40 & 60.44 & 95.18 & 57.19 & 95.76 \\
& MILAN\cite{milan} & 38.54 & 91.01 & 21.01 & 99.36 & 55.26 & 92.75 & 41.81 & 94.67 & 39.16 & 94.45 \\
& CAE\cite{cae} & 51.17 & 94.92 & 52.24 & 94.28 & 52.24 & 94.25 & 52.83 & 94.35 & 52.12 & 94.45 \\
\midrule
\multirow{10}{*}{MaxLogit\cite{maxlogit}}
& ViT\cite{vit} & 67.22 & 77.98 & 89.88 & 45.57 & 61.68 & 88.60 & 82.73 & 62.52 & 75.37 & 68.67 \\
& MoCov3\cite{mocov3} & 62.36 & 77.19 & 90.38 & 42.37 & 65.65 & 82.00 & 84.19 & 54.17 & 75.64 & 63.93 \\
& DINOv2\cite{dinov2} & 54.70 & 86.10 & 69.98 & 85.88 & 45.60 & 96.00 & 54.52 & 93.07 & 56.20 & 90.26 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{\textbf{85.94}} & \cellcolor{gray!20}{46.45} & \cellcolor{gray!20}{\textbf{96.90}} & \cellcolor{gray!20}{\textbf{11.65}} & \cellcolor{gray!20}{83.97} & \cellcolor{gray!20}{48.65} & \cellcolor{gray!20}{\textbf{93.82}} & \cellcolor{gray!20}{\textbf{22.71}} & \cellcolor{gray!20}{\textbf{90.16}} & \cellcolor{gray!20}{32.37} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{84.17} & \cellcolor{gray!20}{\textbf{44.69}} & \cellcolor{gray!20}{96.48} & \cellcolor{gray!20}{13.69} & \cellcolor{gray!20}{\textbf{85.34}} & \cellcolor{gray!20}{\textbf{43.70}} & \cellcolor{gray!20}{93.31} & \cellcolor{gray!20}{23.80} & \cellcolor{gray!20}{89.83} & \cellcolor{gray!20}{\textbf{31.47}} \\
& MaskFeat\cite{maskfeat} & 30.09 & 98.78 & 31.22 & 99.58 & 38.37 & 97.90 & 37.39 & 98.57 & 34.26 & 98.71 \\
& EVA\cite{eva} & 39.11 & 97.17 & 60.53 & 93.45 & 48.32 & 96.20 & 50.72 & 96.02 & 49.67 & 95.71 \\
& MFF\cite{mff} & 42.80 & 96.12 & 50.49 & 95.51 & 51.73 & 94.40 & 57.53 & 92.63 & 50.64 & 94.67 \\
& MILAN\cite{milan} & 40.28 & 93.62 & 27.27 & 99.67 & 56.70 & 93.05 & 43.11 & 94.84 & 41.84 & 95.30 \\
& CAE\cite{cae} & 59.12 & 88.16 & 70.20 & 79.83 & 57.91 & 89.85 & 61.71 & 86.93 & 62.23 & 86.19 \\
\midrule
\multirow{10}{*}{KL-Matching\cite{maxlogit}}
& ViT\cite{vit} & 82.59 & 67.27 & 87.63 & 69.71 & 66.55 & 88.15 & 84.34 & 74.23 & 80.28 & 74.84 \\
& MoCov3\cite{mocov3} & 82.35 & 68.60 & 86.24 & 76.78 & 67.80 & 88.85 & 82.73 & 81.31 & 79.78 & 78.89 \\
& DINOv2\cite{dinov2} & 80.51 & 67.71 & 56.93 & 97.24 & 69.77 & 77.70 & 62.63 & 87.69 & 67.46 & 82.59 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{87.14} & \cellcolor{gray!20}{52.73} & \cellcolor{gray!20}{\textbf{95.13}} & \cellcolor{gray!20}{\textbf{21.94}} & \cellcolor{gray!20}{82.87} & \cellcolor{gray!20}{62.55} & \cellcolor{gray!20}{92.10} & \cellcolor{gray!20}{36.67} & \cellcolor{gray!20}{89.31} & \cellcolor{gray!20}{43.47} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{87.87} & \cellcolor{gray!20}{48.55} & \cellcolor{gray!20}{94.82} & \cellcolor{gray!20}{26.26} & \cellcolor{gray!20}{\textbf{84.56}} & \cellcolor{gray!20}{\textbf{59.65}} & \cellcolor{gray!20}{\textbf{92.48}} & \cellcolor{gray!20}{\textbf{35.70}} & \cellcolor{gray!20}{\textbf{89.93}} & \cellcolor{gray!20}{\textbf{42.54}} \\
& MaskFeat\cite{maskfeat} & 68.52 & 83.10 & 54.66 & 89.41 & 48.18 & 93.35 & 48.65 & 91.45 & 55.00 & 89.33 \\
& EVA\cite{eva} & \textbf{92.47} & \textbf{34.81} & 48.28 & 97.64 & 66.51 & 85.10 & 62.69 & 88.50 & 67.49 & 76.51 \\
& MFF\cite{mff} & 68.06 & 79.03 & 33.42 & 98.95 & 43.85 & 95.35 & 34.26 & 97.18 & 44.90 & 92.63 \\
& MILAN\cite{milan} & 76.45 & 67.58 & 74.07 & 82.24 & 55.70 & 91.30 & 64.51 & 87.07 & 67.68 & 82.05 \\
& CAE\cite{cae} & 61.75 & 90.12 & 36.07 & 98.80 & 47.15 & 96.40 & 42.28 & 97.02 & 46.81 & 95.58 \\
\midrule
\multirow{10}{*}{Residual\cite{vim}}
& ViT\cite{vit} & 82.39 & 64.61 & 73.72 & 86.00 & 68.44 & 87.45 & 74.88 & 77.98 & 74.86 & 79.01 \\
& MoCov3\cite{mocov3} & 75.25 & 76.55 & 73.80 & 83.16 & 57.69 & 92.00 & 67.82 & 86.73 & 68.64 & 84.61 \\
& DINOv2\cite{dinov2} & 66.50 & 72.64 & 61.90 & 97.40 & 58.94 & 87.95 & 56.84 & 90.97 & 61.04 & 87.24 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{94.99} & \cellcolor{gray!20}{\textbf{21.98}} & \cellcolor{gray!20}{99.01} & \cellcolor{gray!20}{4.84} & \cellcolor{gray!20}{87.23} & \cellcolor{gray!20}{58.35} & \cellcolor{gray!20}{95.43} & \cellcolor{gray!20}{24.91} & \cellcolor{gray!20}{94.17} & \cellcolor{gray!20}{27.52} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{94.16} & \cellcolor{gray!20}{25.17} & \cellcolor{gray!20}{\textbf{99.50}} & \cellcolor{gray!20}{\textbf{2.01}} & \cellcolor{gray!20}{\textbf{89.35}} & \cellcolor{gray!20}{\textbf{51.20}} & \cellcolor{gray!20}{\textbf{96.52}} & \cellcolor{gray!20}{\textbf{19.58}} & \cellcolor{gray!20}{\textbf{94.88}} & \cellcolor{gray!20}{\textbf{24.49}} \\
& MaskFeat\cite{maskfeat} & 87.82 & 56.74 & 70.20 & 91.61 & 68.77 & 90.45 & 69.38 & 88.54 & 74.04 & 81.84 \\
& EVA\cite{eva} & \textbf{95.16} & 24.44 & 54.90 & 97.63 & 72.09 & 79.90 & 67.58 & 85.07 & 72.43 & 71.76 \\
& MFF\cite{mff} & 89.50 & 42.19 & 46.18 & 98.55 & 65.70 & 87.00 & 56.57 & 91.83 & 64.49 & 79.89 \\
& MILAN\cite{milan} & 80.63 & 54.22 & 72.92 & 91.80 & 63.76 & 82.70 & 66.46 & 83.08 & 70.94 & 77.95 \\
& CAE\cite{cae} & 70.43 & 87.87 & 38.67 & 98.86 & 50.53 & 96.85 & 44.17 & 97.39 & 50.95 & 95.24 \\
\bottomrule
\end{tabular}
\caption{\textbf{More Masked Image Modeling Methods.} Results of OOD detection methods on ImageNet. Bold ones stand for the best results.}
\label{tab:mim-imagenet}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% second table %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[tp]
\small
\centering
\setlength{\tabcolsep}{0.5mm}
\begin{tabular}{c|c|cccccccccc}
\multirow{2}{*}{Methods} & \multirow{2}{*}{Models} & \multicolumn{2}{c}{Texture} & \multicolumn{2}{c}{iNaturalist} & \multicolumn{2}{c}{ImageNet-O} & \multicolumn{2}{c}{OpenImage-O} & \multicolumn{2}{c}{Average} \\
& & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ \\
\midrule
\multirow{10}{*}{React\cite{react}}
& ViT\cite{vit} & 62.09 & 80.47 & 91.20 & 38.74 & 63.66 & 81.00 & 80.43 & 60.41 & 74.34 & 65.15 \\
& MoCov3\cite{mocov3} & 51.47 & 87.11 & 79.30 & 69.92 & 65.33 & 75.35 & 74.35 & 68.27 & 67.61 & 75.16 \\
& DINOv2\cite{dinov2} & 76.73 & 62.44 & 74.25 & 82.93 & 56.26 & 90.20 & 63.17 & 89.13 & 67.60 & 81.17 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{\textbf{86.10}} & \cellcolor{gray!20}{43.47} & \cellcolor{gray!20}{\textbf{98.09}} & \cellcolor{gray!20}{\textbf{7.01}} & \cellcolor{gray!20}{85.69} & \cellcolor{gray!20}{41.50} & \cellcolor{gray!20}{\textbf{94.96}} & \cellcolor{gray!20}{\textbf{18.09}} & \cellcolor{gray!20}{\textbf{91.21}} & \cellcolor{gray!20}{\textbf{27.52}} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{84.32} & \cellcolor{gray!20}{\textbf{43.41}} & \cellcolor{gray!20}{96.99} & \cellcolor{gray!20}{11.42} & \cellcolor{gray!20}{\textbf{87.04}} & \cellcolor{gray!20}{\textbf{37.60}} & \cellcolor{gray!20}{94.21} & \cellcolor{gray!20}{20.24} & \cellcolor{gray!20}{90.64} & \cellcolor{gray!20}{28.17} \\
& MaskFeat\cite{maskfeat} & 50.57 & 96.49 & 51.17 & 98.12 & 58.57 & 91.55 & 60.07 & 91.92 & 55.10 & 94.52 \\
& EVA\cite{eva} & 39.36 & 95.91 & 53.34 & 98.62 & 57.75 & 89.10 & 56.45 & 93.15 & 51.72 & 94.20 \\
& MFF\cite{mff} & 40.75 & 98.08 & 65.36 & 97.00 & 41.78 & 98.15 & 53.21 & 97.33 & 50.28 & 97.64 \\
& MILAN\cite{milan} & 39.47 & 90.43 & 21.62 & 99.41 & 55.78 & 92.80 & 42.07 & 94.61 & 39.74 & 94.31 \\
& CAE\cite{cae} & 51.97 & 93.60 & 49.55 & 94.71 & 52.77 & 92.85 & 51.49 & 94.36 & 51.44 & 93.88 \\
\midrule
\multirow{10}{*}{Mahalanobis\cite{mahalanobis}}
& ViT\cite{vit} & 84.93 & 66.05 & 84.90 & 81.60 & 71.53 & 88.85 & 84.16 & 74.72 & 81.38 & 77.80 \\
& MoCov3\cite{mocov3} & 84.29 & 68.64 & 86.95 & 76.50 & 70.33 & 90.45 & 83.54 & 79.64 & 81.28 & 78.81 \\
& DINOv2\cite{dinov2} & 68.58 & 71.88 & 63.14 & 97.61 & 58.86 & 87.35 & 57.57 & 90.89 & 62.04 & 86.93 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{93.01} & \cellcolor{gray!20}{30.91} & \cellcolor{gray!20}{98.78} & \cellcolor{gray!20}{5.89} & \cellcolor{gray!20}{86.78} & \cellcolor{gray!20}{63.15} & \cellcolor{gray!20}{95.46} & \cellcolor{gray!20}{26.46} & \cellcolor{gray!20}{93.51} & \cellcolor{gray!20}{31.60} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{93.03} & \cellcolor{gray!20}{30.23} & \cellcolor{gray!20}{\textbf{99.18}} & \cellcolor{gray!20}{\textbf{3.51}} & \cellcolor{gray!20}{\textbf{88.84}} & \cellcolor{gray!20}{\textbf{54.85}} & \cellcolor{gray!20}{\textbf{96.51}} & \cellcolor{gray!20}{\textbf{19.09}} & \cellcolor{gray!20}{\textbf{94.39}} & \cellcolor{gray!20}{\textbf{26.92}} \\
& MaskFeat\cite{maskfeat} & 90.40 & 52.50 & 89.10 & 68.26 & 76.29 & 86.90 & 86.06 & 76.62 & 85.46 & 71.07 \\
& EVA\cite{eva} & \textbf{97.55} & \textbf{12.25} & 77.45 & 92.27 & 79.23 & 70.70 & 81.09 & 74.64 & 83.83 & 62.47 \\
& MFF\cite{mff} & 39.72 & 97.40 & 59.28 & 91.85 & 51.85 & 94.65 & 51.97 & 94.26 & 50.70 & 94.54 \\
& MILAN\cite{milan} & 81.72 & 53.41 & 73.53 & 91.93 & 64.32 & 82.50 & 67.01 & 83.25 & 71.65 & 77.77 \\
& CAE\cite{cae} & 69.95 & 87.97 & 39.17 & 98.74 & 50.27 & 96.35 & 44.36 & 97.11 & 50.94 & 95.04 \\
\midrule
\multirow{10}{*}{ViM\cite{vim}}
& ViT\cite{vit} & 83.51 & 62.71 & 77.75 & 81.72 & 71.04 & 86.60 & 78.31 & 74.55 & 77.65 & 76.40 \\
& MoCov3\cite{mocov3} & 76.28 & 75.72 & 78.18 & 78.82 & 61.35 & 91.50 & 72.46 & 84.12 & 72.07 & 82.54 \\
& DINOv2\cite{dinov2} & 66.90 & 72.21 & 62.53 & 97.19 & 58.93 & 87.90 & 56.93 & 90.85 & 61.32 & 87.04 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{\textbf{95.35}} & \cellcolor{gray!20}{\textbf{21.96}} & \cellcolor{gray!20}{99.31} & \cellcolor{gray!20}{3.18} & \cellcolor{gray!20}{90.06} & \cellcolor{gray!20}{49.85} & \cellcolor{gray!20}{96.96} & \cellcolor{gray!20}{16.80} & \cellcolor{gray!20}{95.42} & \cellcolor{gray!20}{22.95} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{94.25} & \cellcolor{gray!20}{24.69} & \cellcolor{gray!20}{\textbf{99.59}} & \cellcolor{gray!20}{\textbf{1.83}} & \cellcolor{gray!20}{\textbf{91.47}} & \cellcolor{gray!20}{\textbf{40.80}} & \cellcolor{gray!20}{\textbf{97.41}} & \cellcolor{gray!20}{\textbf{13.55}} & \cellcolor{gray!20}{\textbf{95.68}} & \cellcolor{gray!20}{\textbf{20.22}} \\
& MaskFeat\cite{maskfeat} & 87.86 & 56.67 & 70.25 & 91.58 & 68.89 & 90.35 & 69.49 & 88.44 & 74.12 & 81.76 \\
& EVA\cite{eva} & 95.14 & 24.52 & 55.08 & 97.55 & 72.17 & 79.75 & 67.71 & 85.04 & 72.52 & 71.71 \\
& MFF\cite{mff} & 89.51 & 42.11 & 46.38 & 98.54 & 65.69 & 87.00 & 56.67 & 91.83 & 64.56 & 79.87 \\
& MILAN\cite{milan} & 80.02 & 56.24 & 69.91 & 92.85 & 64.90 & 83.20 & 66.19 & 83.96 & 70.25 & 79.06 \\
& CAE\cite{cae} & 70.54 & 87.89 & 38.70 & 98.87 & 50.59 & 96.85 & 44.24 & 97.36 & 51.02 & 95.24 \\
\midrule
\multirow{10}{*}{Average}
& ViT\cite{vit} & 73.52 & 72.81 & 84.05 & 64.97 & 65.66 & 86.53 & 80.02 & 70.03 & 75.81 & 73.58 \\
& MoCov3\cite{mocov3} & 68.45 & 77.30 & 82.79 & 67.83 & 64.69 & 85.04 & 77.83 & 72.40 & 73.44 & 75.64 \\
& DINOv2\cite{dinov2} & 66.91 & 74.11 & 66.40 & 88.72 & 55.40 & 89.61 & 57.64 & 90.46 & 61.59 & 85.72 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{\textbf{89.18}} & \cellcolor{gray!20}{39.14} & \cellcolor{gray!20}{\textbf{97.53}} & \cellcolor{gray!20}{\textbf{10.26}} & \cellcolor{gray!20}{85.38} & \cellcolor{gray!20}{52.91} & \cellcolor{gray!20}{94.42} & \cellcolor{gray!20}{24.45} & \cellcolor{gray!20}{91.63} & \cellcolor{gray!20}{31.69} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{88.24} & \cellcolor{gray!20}{\textbf{38.77}} & \cellcolor{gray!20}{97.32} & \cellcolor{gray!20}{11.34} & \cellcolor{gray!20}{\textbf{87.02}} & \cellcolor{gray!20}{\textbf{47.58}} & \cellcolor{gray!20}{\textbf{94.53}} & \cellcolor{gray!20}{\textbf{23.03}} & \cellcolor{gray!20}{\textbf{91.77}} & \cellcolor{gray!20}{\textbf{30.18}} \\
& MaskFeat\cite{maskfeat} & 63.29 & 79.34 & 56.50 & 91.83 & 57.44 & 92.28 & 58.63 & 90.69 & 58.96 & 88.54 \\
& EVA\cite{eva} & 69.58 & 58.63 & 59.25 & 95.70 & 63.43 & 85.82 & 62.62 & 88.56 & 63.72 & 82.18 \\
& MFF\cite{mff} & 57.68 & 80.94 & 52.74 & 96.28 & 52.66 & 93.54 & 53.48 & 94.13 & 54.14 & 91.22 \\
& MILAN\cite{milan} & 59.92 & 75.06 & 49.05 & 94.62 & 59.14 & 88.80 & 54.42 & 89.55 & 55.63 & 87.01 \\
& CAE\cite{cae} & 61.77 & 89.82 & 49.37 & 92.94 & 52.42 & 94.19 & 50.35 & 93.90 & 53.48 & 92.71 \\
\midrule
\multirow{10}{*}{Best}
& ViT\cite{vit} & 84.93 & 62.71 & 91.20 & 38.74 & 71.53 & 81.00 & 84.34 & 60.41 & 81.38 & 65.15 \\
& MoCov3\cite{mocov3} & 84.29 & 68.60 & 90.68 & 42.03 & 70.33 & 75.35 & 85.42 & 54.17 & 81.28 & 63.93 \\
& DINOv2\cite{dinov2} & 80.51 & 62.44 & 80.34 & 59.18 & 69.77 & 77.70 & 63.17 & 87.03 & 67.60 & 77.13 \\
& \cellcolor{gray!20}{BEiTv2\cite{beitv2}} & \cellcolor{gray!20}{95.35} & \cellcolor{gray!20}{21.96} & \cellcolor{gray!20}{99.31} & \cellcolor{gray!20}{3.18} & \cellcolor{gray!20}{90.06} & \cellcolor{gray!20}{40.95} & \cellcolor{gray!20}{96.96} & \cellcolor{gray!20}{16.80} & \cellcolor{gray!20}{95.42} & \cellcolor{gray!20}{22.95} \\
& \cellcolor{gray!20}{BEiT\cite{beit} } & \cellcolor{gray!20}{94.25} & \cellcolor{gray!20}{24.69} & \cellcolor{gray!20}{\textbf{99.59}} & \cellcolor{gray!20}{\textbf{1.83}} & \cellcolor{gray!20}{\textbf{91.47}} & \cellcolor{gray!20}{\textbf{37.60}} & \cellcolor{gray!20}{\textbf{97.41}} & \cellcolor{gray!20}{\textbf{13.55}} & \cellcolor{gray!20}{\textbf{95.68}} & \cellcolor{gray!20}{\textbf{20.22}} \\
& MaskFeat\cite{maskfeat} & 90.40 & 52.50 & 89.10 & 68.26 & 76.29 & 86.90 & 86.06 & 76.62 & 85.46 & 71.07 \\
& EVA\cite{eva} & \textbf{97.55} & \textbf{12.25} & 77.45 & 92.27 & 79.23 & 70.70 & 81.09 & 74.64 & 83.83 & 62.47 \\
& MFF\cite{mff} & 89.51 & 42.11 & 71.22 & 91.85 & 65.70 & 87.00 & 60.44 & 91.83 & 64.56 & 79.87 \\
& MILAN\cite{milan} & 81.72 & 53.41 & 74.07 & 82.24 & 64.90 & 82.50 & 67.01 & 83.08 & 71.65 & 77.77 \\
& CAE\cite{cae} & 70.54 & 87.87 & 70.37 & 79.43 & 57.94 & 89.85 & 61.74 & 86.72 & 62.32 & 86.06 \\
\bottomrule
\end{tabular}
\caption{\textbf{More Masked Image Modeling Methods} (continue). Results of OOD detection methods on ImageNet. Bold ones stand for the best results.}
\label{tab:mim-imagenet-continue}
\end{table*}

==> tables/multi-class-cifar10-avgood.tex <==
%%%%%%%%%%%%%%% two tables %%%%%%%%%%%%%%%
\iffalse
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{2.5mm}
\begin{tabular}{c|cccccccccccc}
\toprule
% Models & MSP\cite{baseline_ood} & Energy\cite{energy} & MaxLogit\cite{maxlogit} & KL-Matching\cite{maxlogit} & Residual & React\cite{react} & Mahalanobis\cite{mahalanobis} & ViM\cite{vim} & Best \\
Models & MSP & Energy & MaxLogit & KL-Matching & Residual & Energy+React & Mahalanobis & ViM & Best \\
\midrule
ViT\cite{vit} & 52.25 & 40.65 & 49.56 & 94.97 & 99.59 & 48.94 & 99.31 & 99.63 & 99.63 \\
MoCov3\cite{mocov3} & 47.28 & 37.92 & 44.92 & 94.64 & 99.65 & 38.52 & 99.35 & 99.73 & 99.73 \\
DINOv2\cite{dinov2} & \textbf{76.59} & \textbf{80.20} & \textbf{80.40} & \textbf{97.82} & 99.98 & 54.22 & \textbf{99.99} & \textbf{99.98} & 99.99 \\
\rowcolor{gray!20}BEiTv2\cite{beitv2} & 66.24 & 74.95 & 70.79 & 93.67 & 99.92 & \textbf{75.55} & 99.84 & 99.87 & 99.92 \\
\rowcolor{gray!20}BEiT\cite{beit} & 59.68 & 67.10 & 62.99 & 95.33 & \textbf{99.99} & 67.18 & 99.98 & 99.98 & \textbf{99.99} \\
\bottomrule
\end{tabular}
\caption{\textbf{Multi-Class OOD Detection on CIFAR-10.} AUROC (\%) of multi-class OOD Detection on CIFAR-10.}
\label{tab:multi-cifar10-auroc}
\end{table*}

\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{2.5mm}
\begin{tabular}{c|cccccccccccc}
\toprule
% Models & MSP\cite{baseline_ood} & Energy\cite{energy} & MaxLogit\cite{maxlogit} & KL-Matching\cite{maxlogit} & Residual & React\cite{react} & Mahalanobis\cite{mahalanobis} & ViM\cite{vim} & Best \\
Models & MSP & Energy & MaxLogit & KL-Matching & Residual & Energy+React & Mahalanobis & ViM & Best \\
\midrule
ViT\cite{vit} & 91.81 & 97.50 & 93.43 & 26.71 & 1.49 & 93.76 & 2.47 & 1.39 & 1.39 \\
MoCov3\cite{mocov3} & 94.83 & 97.04 & 95.78 & 30.30 & 1.38 & 97.05 & 2.84 & 0.99 & 0.99 \\
DINOv2\cite{dinov2} & \textbf{52.73} & \textbf{41.15} & \textbf{42.61} & \textbf{9.99} & 0.07 & 80.87 & 0.05 & 0.07 & 0.05 \\
\rowcolor{gray!20}BEiTv2\cite{beitv2} & 76.03 & 61.24 & 69.98 & 36.24 & 0.30 & \textbf{58.30} & 0.69 & 0.51 & 0.30 \\
\rowcolor{gray!20}BEiT\cite{beit} & 84.17 & 71.34 & 79.74 & 27.78 & \textbf{0.03} & 71.03 & \textbf{0.03} & \textbf{0.07} & \textbf{0.03} \\
\bottomrule
\end{tabular}
\caption{\textbf{Multi-Class OOD Detection on CIFAR-10.} FPR95 (\%) of multi-class OOD Detection on CIFAR-10.}
\label{tab:multi-cifar10-fpr50}
\end{table*}
\fi

%%%%%%%%%%%%%%% one tables %%%%%%%%%%%%%%%
\begin{table*}[t]
\small
\centering
\subfloat[AUROC]{
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{c|cccccccccccc}
\toprule
% Models & MSP\cite{baseline_ood} & Energy\cite{energy} & MaxLogit\cite{maxlogit} & KL-Matching\cite{maxlogit} & Residual & React\cite{react} & Mahalanobis\cite{mahalanobis} & ViM\cite{vim} & Best \\
Models  & MSP & Energy & MaxLogit & KL-Matching & Residual & Energy+React & Mahalanobis & ViM & Average & Best \\
\midrule
ViT\cite{vit} & 52.25 & 40.65 & 49.56 & 94.97 & 99.59 & 48.94 & 99.31 & 99.63 & 73.11 & 99.63 \\
MoCov3\cite{mocov3} & 47.28 & 37.92 & 44.92 & 94.64 & 99.65 & 38.52 & 99.35 & 99.73 & 70.25 & 99.73 \\
DINOv2\cite{dinov2} & \textbf{76.59} & \textbf{80.20} & \textbf{80.40} & \textbf{97.82} & 99.98 & 54.22 & \textbf{99.99} & \textbf{99.98} & \textbf{86.15} & 99.99 \\
\rowcolor{gray!20}BEiTv2\cite{beitv2} & 66.24 & 74.95 & 70.79 & 93.67 & 99.92 & \textbf{75.55} & 99.84 & 99.87 & 85.11 & 99.92 \\
\rowcolor{gray!20}BEiT\cite{beit} & 59.68 & 67.10 & 62.99 & 95.33 & \textbf{99.99} & 67.18 & 99.98 & 99.98 & 81.53 & \textbf{99.99} \\
\bottomrule
\end{tabular}
\label{tab:multi-cifar10-avgood-auroc}
}

\subfloat[FPR95]{
\setlength{\tabcolsep}{1.5mm}
\begin{tabular}{c|cccccccccccc}
\toprule
% Models & MSP\cite{baseline_ood} & Energy\cite{energy} & MaxLogit\cite{maxlogit} & KL-Matching\cite{maxlogit} & Residual & React\cite{react} & Mahalanobis\cite{mahalanobis} & ViM\cite{vim} & Best \\
Models & MSP & Energy & MaxLogit & KL-Matching & Residual & Energy+React & Mahalanobis & ViM & Average & Best \\
\midrule
ViT\cite{vit} & 91.81 & 97.50 & 93.43 & 26.71 & 1.49 & 93.76 & 2.47 & 1.39 & 51.07 & 1.39 \\
MoCov3\cite{mocov3} & 94.83 & 97.04 & 95.78 & 30.30 & 1.38 & 97.05 & 2.84 & 0.99 & 52.53 & 0.99 \\
DINOv2\cite{dinov2} & \textbf{52.73} & \textbf{41.15} & \textbf{42.61} & \textbf{9.99} & 0.07 & 80.87 & 0.05 & 0.07 & \textbf{28.44} & 0.05 \\
\rowcolor{gray!20}BEiTv2\cite{beitv2} & 76.03 & 61.24 & 69.98 & 36.24 & 0.30 & \textbf{58.30} & 0.69 & 0.51 & 37.91 & 0.30 \\
\rowcolor{gray!20}BEiT\cite{beit} & 84.17 & 71.34 & 79.74 & 27.78 & \textbf{0.03} & 71.03 & \textbf{0.03} & \textbf{0.07} & 41.77 & \textbf{0.03} \\
\bottomrule
\end{tabular}
\label{tab:multi-cifar10-avgood-fpr50}
}
\caption{\textbf{Multi-Class OOD Detection on CIFAR-10.} Performance of multi-class OOD Detection on CIFAR-10.}
\label{tab:multi-cifar10-avgood}
\end{table*}

==> tables/one-class-avgood.tex <==
\begin{table*}[t]
\small
\centering
\setlength{\tabcolsep}{0.7mm}
\begin{tabular}{c|cccccccccccc}
\toprule
Methods & \multicolumn{2}{c}{KL-Matching\cite{maxlogit}} & \multicolumn{2}{c}{Residual} & \multicolumn{2}{c}{Mahalanobis\cite{mahalanobis}} & \multicolumn{2}{c}{ViM\cite{vim}} & \multicolumn{2}{c}{Average} & \multicolumn{2}{c}{Best} \\
Models & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ & AUROC$\uparrow$ & FPR95$\downarrow$ \\
\midrule
ViT\cite{vit} & 92.11 & 32.96 & 94.58 & 24.82 & 94.64 & 25.34 & 94.63 & 24.63 & 69.56 & 63.32 & 94.64 & 24.63 \\
MoCov3\cite{mocov3} & 89.91 & 42.39 & 94.90 & 24.20 & 94.50 & 26.71 & 95.20 & 22.94 & 69.40 & 65.00 & 95.20 & 22.94 \\
DINOv2\cite{dinov2} & 62.41 & 87.06 & 66.85 & 85.25 & 67.04 & 84.76 & 66.90 & 85.26 & 57.03 & 89.60 & 67.04 & 84.76 \\
\rowcolor{gray!20}BEiTv2\cite{beitv2} & \textbf{96.30} & \textbf{14.58} & 98.39 & \textbf{7.61} & 98.51 & \textbf{7.15} & 97.68 & 10.33 & \textbf{71.21} & \textbf{54.55} & 98.51 & \textbf{7.15} \\
\rowcolor{gray!20}BEiT\cite{beit} & 95.13 & 19.80 & \textbf{98.46} & 8.44 & \textbf{98.57} & 7.80 & \textbf{98.20} & \textbf{9.49} & 71.16 & 54.68 & \textbf{98.57} & 7.80 \\
\bottomrule
\end{tabular}
\caption{\textbf{One-Class OOD Detection.} AUROC (\%) of one-class OOD Detection.}
\label{tab:one-class-avgood}
\end{table*}
